Robo-AO Kepler Planetary Candidate Survey II: Adaptive Optics Imaging of 969 Kepler Exoplanet Candidate Host Stars

We initiated the Robo-AO Kepler Planetary Candidate Survey in 2012 to observe each Kepler exoplanet candidate host star with high-angular-resolution visible-light laser-adaptive-optics imaging. Our goal is to find nearby stars lying in Kepler's photometric apertures that are responsible for the relatively high probability of false-positive exoplanet detections and that cause underestimates of the size of transit radii. Our comprehensive survey will also shed light on the effects of stellar multiplicity on exoplanet properties and will identify rare exoplanetary architectures. In this second part of our ongoing survey, we observed an additional 969 Kepler planet candidate hosts and we report blended stellar companions up to $\Delta m \approx 6$ that contribute to Kepler's measured light curves. We found 203 companions within $\sim$4" of 181 of the Kepler stars, of which 141 are new discoveries. We measure the nearby-star probability for this sample of Kepler planet candidate host stars to be 10.6% $\pm$ 1.1% at angular separations up to 2.5", significantly higher than the 7.4% $\pm$ 1.0% probability discovered in our initial sample of 715 stars; we find the probability increases to 17.6% $\pm$ 1.5% out to a separation of 4.0". The median position of KOIs observed in this survey are 1.1$^{\circ}$ closer to the galactic plane which may account for some of the nearby-star probability enhancement. We additionally detail 50 Keck adaptive optics images of Robo-AO observed KOIs in order to confirm 37 companions detected at a $<5\sigma$ significance level and to obtain additional infrared photometry on higher-significance detected companions.

==> big_figures.tex <==

%----------------------------------------------------------------------------------------------------------
\begin{figure*}
\centering
\includegraphics[width=500pt]{koi2_binaries_grid1.pdf}
\caption{Color inverted, normalized log-scale cutouts of 61 multiple KOI systems [KOI-4 to KOI-2056] with separations $<$4$\arcsec$ resolved with Robo-AO.  The angular scale and orientation is similar for each cutout.  The smaller circles are centered on the detected nearby star.}
\label{fig:cutouts1}
\end{figure*}
%----------------------------------------------------------------------------------------------------------


%----------------------------------------------------------------------------------------------------------
\begin{figure*}
\centering
\includegraphics[width=500pt]{koi2_binaries_grid2.pdf}
\caption{Color inverted, normalized log-scale cutouts of 61 multiple KOI systems [KOI-2067 to KOI-3277] with separations $<$4$\arcsec$ resolved with Robo-AO.  The angular scale and orientation is similar for each cutout.  The smaller circles are centered on the detected nearby star.}
\label{fig:cutouts2}
\end{figure*}
%----------------------------------------------------------------------------------------------------------


%----------------------------------------------------------------------------------------------------------
\begin{figure*}
\centering
\includegraphics[width=500pt]{koi2_binaries_grid3.pdf}
\caption{Color inverted, normalized log-scale cutouts of \textbf{59} multiple KOI systems [KOI-3284 to KOI-4871] with separations $<$4$\arcsec$ resolved with Robo-AO.  The angular scale and orientation is similar for each cutout.  The smaller circles are centered on the detected nearby star.}
\label{fig:cutouts3}
\end{figure*}
%----------------------------------------------------------------------------------------------------------


